High Rate Studies of the ATLAS sTGC Detector and Optimization of the Filter Circuit on the Input of the Front-End Amplifier

The Large Hadron Collider (LHC) at CERN is expected to be upgraded to the High-Luminosity LHC (HL-LHC) by 2029 and achieve instantaneous luminosity around 5 - 7.5 $\times$ 10$^{34}$cm$^{-2}$ s$^{-1}$. This represents a more than 3-4 fold increase in the instantaneous luminosity compared to what has been achieved in Run 2. The New Small Wheel (NSW) upgrade is designed to be able to operate efficiently in this high background rate environment. In this article, we summarize multiple performance studies of the small-strip Thin Gap Chamber (sTGC) at high rate using nearly final front-end electronics. We demonstrate that the efficiency versus rate distribution can be well described by an exponential decay with electronics dead-time being the primary cause of loss of efficiency at high rate. We then demonstrate several methods that can decrease the electronics dead-time and therefore minimize efficiency loss. One such method is to install either a pi-network input filter or pull-up resistor to minimize the charge input into the amplifier. We optimized the pi-network capacitance and pull-up resistor resistance using the results from our measurements. The results shown here were not only critical to finalizing the components on the front-end board, but also are critical for setting the optimal operating parameters of the sTGC detector and electronics in the ATLAS cavern.

==> section_detector_emulator.tex <==
\section{Detector emulation}
\label{sec: detector emulation}
In this section we present the methodology and results of detector emulation studies aimed at characterizing the VMM3a chip performance by means of a realistic sTGC signal. In this way we could investigate ina controlled way the causes for VMM3a dead time described above, namely the recovery of the analog baseline and the digitization time. 

We focused in particular on a pad-like condition, trying to test different values of the $\uppi$-network capacitor for each pad-equivalent capacitance. We could reproduce the muon spectrum and the detection efficiency in different points of the parameter space. We also tried different VMM3a bits configuration and we tested the case when no external pull-up current is provided. With this method we could test the electronics up to an emulated photon rate of $\sim$1~MHz.
This work was conducted at Technion.

\subsection{Detector emulator technique}
\label{subsec: detector emulator technique}
A current pulse which shape closely resembles that of a sTGC detector was inputted into the VMM3a chip by means of an injection circuit, depicted in figure~\ref{subfig: injector circuit}. The injection circuit operates on it's input voltage signal as a mathematical derivative, as it can be seen from the LTspice simulation results in figure~\ref{subfig: LTspice simulation}. For this reason, the input to the injector must be the integral as a function of time of the current pulse induced in a real detector. The operation can be described by the formula $i(t) \sim \frac{d}{dt}V(t)$, where V(t) is the injector input - e.g. a signal recorded by means of a charge sensitive preamplifier with long decay time -, the time derivative is the injector operation, and i(t) is the injector output entering the VMM3a. The details of the detector emulator signals that were used in this work are given in appendix~\ref{app: det emulator input}. The injector input waveforms were played by the Analog Waveform Generator (AWG) machines \href{https://www.caen.it/products/dt5800/}{CAEN DT5800} and \href{https://www.keysight.com/il/en/products/arbitrary-waveform-generators/m8100-series-arbitrary-waveform-generators.html}{Keysight AWG M8190A}, each of them connected to a separate injector channel. The CAEN module is capable of producing waveforms with a custom shape, random pulse heights drawn from a custom distribution, and random times (exponential) at a set average rate. The machine has 16 memories available for signal pileup, providing a maximum rate of $\sim$1/(16$~\times~signal~duration$). For the used signal shape (see appendix~\ref{app: det emulator input}) the rate limit was $\sim$40~kHz. The CAEN DT5800 was used to inject directly $\upmu$-like signals at 1kHz constant rate, but also to record input waveforms for the Keysight module: sequences of $\upgamma$-like signals produced at random times at the maximum possible average rate, were added to effectively increase the signal rate. Notice that the difference between $\upgamma$ and $\upmu$ waveforms was the charge spectrum and timing of the signals, while the signal shape was the same for both cases. 
We could set the injected pulses height distribution to reproduce the one measured in the October test beam in GIF++ with a QL1 prototype, both for photons ($\upgamma$) and muons ($\upmu$). The $\upmu$ rate was kept constant at 1~kHz, while the $\upgamma$ signals were reproduced at random times (exponential) at different average rates up to $\sim$1~MHz. 
In order to mimic the real sTGC pad capacitance, an extra capacitor ($\mathrm{C_{pad}}$) was introduced in the circuit, together with the $\uppi$-network scheme (figure~\ref{fig: pi-network}). The tested \cpad~ values were 800~pF and 2~nF (close to the measured pad capacitance for QL1 and QS3 sTGC modules, respectively). Table~\ref{tab: parameter space} summarizes the explored parameter space and the theoretical attenuation factor for each combination of capacitances, according to the formula $f_{att}= \cpi/(\cpi+\cpad)$.


\begin{table}[h]
\begin{center}
\begin{tabular}{| c | c | c |}
\hline
\textbf{\cpad~[pF]} & \textbf{\cpi~[pF]} & \textbf{attenuation factor}\\ \hline
\multirow{4}{*}{800} & 100 & 0.1 \\ \cline{2-3}
& 200 & 0.2 \\ \cline{2-3}
& 300 & 0.27 \\ \cline{2-3}
& 470 & 0.37 \\ \hline
\multirow{5}{*}{2000} & 200 & 0.9 \\ \cline{2-3}
& 470 & 0.19 \\ \cline{2-3}
& 600 & 0.23 \\ \cline{2-3}
& 800 & 0.29 \\ \cline{2-3}
& 1000 & 0.33 \\ \hline
\end{tabular}
\caption{The explored parameter space.}
\label{tab: parameter space}
\end{center}
\end{table}

\begin{figure}[htbp]
\centering
\subfloat[The current injector scheme]{
\includegraphics[scale=0.3]{figures/emulator/injector_circuit.png}
\label{subfig: injector circuit}
}
\subfloat[LTspice simulation of the injector]{
\includegraphics[scale=0.42]{figures/emulator/injector_simulation.png}
\label{subfig: LTspice simulation}
}
\caption{The current injector scheme is shown in~\protect\subref{subfig: injector circuit}. For each of the two channels working independently: a voltage pulse (V) is injected into a capacitor (C), which is connected to the electronics input (R$\mathrm{_{VMM}}$ - it is not part of the injector). A LTspice simulation~\protect\subref{subfig: LTspice simulation} shows the normalized injector output for a wide range of C values, demonstrating that it resembles the mathematical derivative of the input voltage.  
}
\label{fig: injector}
\end{figure}

\begin{figure}[htbp]
\centering
\subfloat[The current injector scheme with $\uppi$-network]{
\includegraphics[scale=0.3]{figures/emulator/pi_network_circuit.png}
\label{subfig: pi-network circuit}
}
\subfloat[The current injector circuit with $\uppi$-network]{
\includegraphics[scale=0.42]{figures/emulator/pi-network.png}
\label{subfig: pi-network}
}
\caption{\protect\subref{subfig: pi-network circuit} The current injector described in~\ref{fig: injector} is connected to a $\uppi$-network circuit. An additional capacitor (\cpad) represents the capacitance of a sTGC pad. Both values of \cpad~and \cpi~can be changed. The actual device is shown in \protect\subref{subfig: pi-network}.
}
\label{fig: pi-network}
\end{figure}

The VMM3a chip was installed onto a GPVMM board~\cite{gkountoumis2018prototype}, from which it is possible to readout both analog and digital outputs. Analog outputs and the 1-bit digital output ("direct output") were monitored and recorded from an oscilloscope, while the 10-bit ADC output was recorded from a PC by the VERSO DAQ software~\cite{verso}.
The parameters of the VMM3a chip were fixed to the values reported in figure~\ref{fig: emulator VMM3a config}, unless specified for particular measurements.

\begin{figure}[htbp]
\centering
\subfloat[\cpad= 800~pF]{
\includegraphics[scale=0.15]{figures/emulator/VMM_config_1.png}
}
\subfloat[\cpad= 2~nF]{
\includegraphics[scale=0.15]{figures/emulator/VMM_config_2.png}
}
\caption{VMM3a configuration used in the detector emulator study.
}
\label{fig: emulator VMM3a config}
\end{figure}

\subsection{Measurements and results}
\label{subsec: detector emulator measurements and results}

\subsubsection{Parameter space starting point and emulated spectra}
\label{subsubsec: emulated spectra}

The emulator configuration \cpad= 800~pF, \cpi= 100~pF, was taken as initial point in the parameter space to fix the AWG spectra.
We set the emulator \ph~ and \muon~ pulse height distributions to reproduce those measured in GIF++ at a sTGC voltage of 2900~V under \ph~ rate of $\sim$400~kHz in the considered pad (see section~\ref{sec: TB October}). In this way the voltage drop (i.e. gain drop) caused by the current flowing through the wires is taken into account for a reasonably high \ph~ rate. The emulated \muon~spectrum reproduces well the original one, as shown in figure~\ref{fig: starting point mu}. In order to obtain the correct fraction of saturated events, the tail of the emulated charge distribution was cut at 12~MPV. Figure~\ref{fig: starting point ph} presents the measured and emulated \ph~ spectra. In this case it was not possible to reproduce the measured fraction of saturated events, due to the limited dynamic range of the AWG. Moreover, the emulated \ph~ spectra at high rate show some extra noise, due to the method described in section~\ref{sec: detector emulation}, which requires adding together several waveforms. This is taken care of when we set the threshold for each efficiency measurement, as described in section~\ref{subsubsec: efficiency measurement}. 

After setting the starting point, the parameter space was explored by changing the values of \cpad~ and \cpi~ and the VMM3a bits.
The \muon~ and \ph~ spectra obtained with different \cpi~ values are presented in figures~\ref{fig: spectra muons} and~\ref{fig: spectra ph}, respectively for \cpad= 800~pF and \cpad= 2~nF. It can be seen that the most probable value (MPV) of the distributions changes according to the attenuation factors summarized in table~\ref{tab: parameter space}.

\begin{figure}[htbp]
\centering
\subfloat[\muon~ spectrum from test beam]{
\includegraphics[scale=0.5]{figures/emulator/starting_point_TB.png}
\label{subfig: starting point TB mu}
}
\subfloat[Emulated \muon~ spectrum]{
\includegraphics[scale=0.5]{figures/emulator/starting_point_emu.png}
\label{subfig: starting point emu mu}
}
\caption{VMM3a 10-bit ADC readout: \protect\subref{subfig: starting point TB mu} \muon~spectrum recorded from sTGC QL1 operated at 2900~V in GIF++ under $\sim$400~kHz \ph~background rate. \protect\subref{subfig: starting point emu mu} Emulated \muon~ spectrum used as initial point in the parameter space.}
\label{fig: starting point mu}
\end{figure}

\begin{figure}[htbp]
\centering
\subfloat[\ph~ spectrum from test beam]{
\includegraphics[scale=0.5]{figures/emulator/TB_ph_spectrum.png}
\label{subfig: starting point TB ph}
}
\subfloat[Emulated \ph~ spectrum]{
\includegraphics[scale=0.5]{figures/emulator/emulated_ph_spectrum.png}
\label{subfig: starting point emu ph}
}
\caption{VMM3a 10-bit ADC readout: \protect\subref{subfig: starting point TB ph} $\sim$400~kHz background \ph~spectrum recorded from sTGC QL1 operated at 2900~V in GIF++. \protect\subref{subfig: starting point emu ph} Emulated \ph~ spectra at different rates. \muon~spectra are also shown for comparison.
}
\label{fig: starting point ph}
\end{figure}


\begin{figure}[htbp]
\centering
\subfloat[\cpad= 800~pF]{
\includegraphics[scale=0.5]{figures/emulator/emulated_spectra_800pf.png}
\label{subfig: spectra QL1}
}
\subfloat[\cpad= 2~nF]{
\includegraphics[scale=0.5]{figures/emulator/emulated_spectra_2nf.png}
\label{subfig: spectra QS3}
}
\caption{VMM3a 10-bit ADC readout: Emulated \muon~ spectra for different values of \cpi, for \cpad= 800~pF \protect\subref{subfig: spectra QL1} and \cpad= 2~nF  \protect\subref{subfig: spectra QS3}.
}
\label{fig: spectra muons}
\end{figure}

\begin{figure}[htbp]
\centering
\subfloat[\cpad= 800~pF]{
\includegraphics[scale=0.56]{figures/emulator/emulated_spectra_ph.png}
\label{subfig: spectra ph QL1}
}
\subfloat[\cpad= 2~nF]{
\includegraphics[scale=0.5]{figures/emulator/emulated_spectra_ph_2nF.png}
\label{subfig: spectra ph QS3}
}
\caption{VMM3a 10-bit ADC readout: Emulated \ph~ spectra for different values of \cpi, for \cpad= 800~pF \protect\subref{subfig: spectra ph QL1} and \cpad= 2~nF  \protect\subref{subfig: spectra ph QS3}.
}
\label{fig: spectra ph}
\end{figure}

\subsubsection{Efficiency measurement}
\label{subsubsec: efficiency measurement}

The effect of the \ph~ background rate on the \muon~ detection efficiency was tested at different points of the parameter space.
The \muon~detection efficiency was defined by means of a 20~ns acceptance window, generated simultaneously with every \muon~ event.
The coincidence between the VMM3a 1-bit output in pulse-at-peak (PtP) mode and the acceptance window determines the efficiency of the event. Effectively, this is like testing a 45~ns time window. 
In spite of the fact that the 1-bit representation should not affect much the VMM3a operation itself, it is important to use PtP output mode (and not time-over-threshold for example) to estimate correctly the inefficiency caused by the chip recovery time. As described above, the VMM3a digital output is ready to accept new signals only after an idle time caused by the re-arming (analog signal returning below threshold) plus a fixed digitization time which is measured to be $\sim$60~ns (larger than the theoretical value of 30~ns) and can reach $\sim$200~ns in case that the 10-bit digitization is active.  
An example of efficient isolated \muon~ event is depicted in figure~\ref{fig: efficiency definition}. In case that the \ph~ background is played, the picture gets more complicated, and more sources of inefficiency (other than signal below threshold) come into play. A summary of possible causes of inefficiency is given in figure~\ref{fig: inefficiency causes}. When a \ph~ comes just before a \muon~ and the two induced signals merge (pileup) so that the voltage does not go below threshold, the event is inefficient because the VMM3a digitizer is not re-armed (figure~\ref{subfig: cause1 pileup}). An event can also be inefficient because of jitter. In the present emulation the intrinsic sTGC signal jitter is not included, whereas there is a jitter component caused by the \ph~ background (figure~\ref{subfig: cause2 jitter}). Other than jitter, the digital output and the acceptance window can be mismatched because of deep saturation of the analog signal, causing the peak to be detected at the wrong time (figure~\ref{subfig: cause3 deepsat}). It is also important to note that deeply saturated signals have a long tail, which can remain above threshold for several $\upmu$s (figure~\ref{subfig: cause3 deepsat}). The time extension of the tail increases with the amount of charge in the pulse. On top of that, when a second signal comes close enough to the tail, it merges with it causing an extra extension. This phenomenon is depicted in figure~\ref{fig: tail extension} using the 1-bit ToT mode.

From this description it results that the amount of deeply saturated events is a cause of harsh inefficiency. Within the linear range of the chip, instead, the spectrum shape affects the efficiency mainly because of the ToT. In particular, in case that the spectrum is scaled by a factor, without changing the threshold, the ToT will increase. In order to minimize the ToT effect and to have a fair comparison between measurements, the threshold should be always set at a fixed value with respect to the spectrum shape (e.g. at the beginning of the Landau distribution), so that the time-over-threshold remains similar. For this reason the threshold for each point in the parameter space was set so that the measured \muon~ efficiency with no \ph~ background was 98$\%$. 

The results of the efficiency measurements are presented in figure~\ref{fig: efficiency_results}. The photon rate was obtained by counting the rate of VMM3a 1-bit outputs and dividing by the measured inefficiency. It can be seen that for both the QL1- and the QS3-like cases the efficiency curve does not change significantly until the attenuation factor reaches $\sim$0.3 (table~\ref{tab: parameter space}). This confirms the hypothesis that the dominant factor causing a worse efficiency is the increased fraction of deeply saturated events, whereas in the linear range the details of the spectrum shape are less important. Applying an exponential fit to curves corresponding to an attenuation factor <0.3, we can extract the average dead time (according to formula~\ref{eqn: efficiency_exponential}), which is $\sim$240~ns and $\sim$280~ns for QL1 and QS3, respectively. 
Measurements with different VMM3a bits configurations are shown in figure~\ref{fig: efficiency bits}. In the same plot we show a measurement without pull-up current. In all the tested cases there was no appreciable difference in the measured efficiency trend.

\begin{figure}[htbp]
\centering
\includegraphics[scale=0.4]{figures/emulator/effficiency_def.png}
\caption{Example of efficient \muon~ event: the analog VMM3a signal (Yellow) passes the threshold (Orange), causing a pulse at the peak time in the 1-bit output (Green). The coincidence between the 1-bit output and the acceptance window (Red) determines the efficiency of the event.
}
\label{fig: efficiency definition}
\end{figure}

\begin{figure}[htbp]
\centering
\subfloat[Pileup]{
\includegraphics[scale=0.35]{figures/emulator/cause1_pileup.png}
\label{subfig: cause1 pileup}
}
\subfloat[Jitter]{
\includegraphics[scale=0.4]{figures/emulator/cause2_jitter.png}
\label{subfig: cause2 jitter}
}
\subfloat[Deep saturation]{
\includegraphics[scale=0.4]{figures/emulator/cause3_deepsat.png}
\label{subfig: cause3 deepsat}
}
\caption{Possible causes of \muon~ detection inefficiency.
}
\label{fig: inefficiency causes}
\end{figure}

\begin{figure}[htbp]
\centering
\subfloat[]{
\includegraphics[scale=0.23]{figures/emulator/tail_merging_1.png}
}
\subfloat[]{
\includegraphics[scale=0.23]{figures/emulator/tail_merging_2.png}
}
\subfloat[]{
\includegraphics[scale=0.23]{figures/emulator/tail_merging_3.png}
}
\caption{A second signal merging to the tail of a deeply saturated one.
}
\label{fig: tail extension}
\end{figure}


\begin{figure}[htbp]
\centering
\subfloat[]{
\includegraphics[scale=0.5]{figures/emulator/efficiency_QL1.png}
\label{subfig: eff_QL1}
}
\subfloat[]{
\includegraphics[scale=0.5]{figures/emulator/efficiency_QS_3.png}
\label{subfig: eff_QS3}
}
\caption{Emulated \muon~ detection efficiency as a function of the \ph~ background rate for different values of \cpi~ , for \cpad~ close to the QL1 (\protect\subref{subfig: eff_QL1}) and QS3 (\protect\subref{subfig: eff_QS3}) prototype values. Exponential fits are also shown.
}
\label{fig: efficiency_results}
\end{figure}

\begin{figure}[htbp]
\centering
\includegraphics[scale=0.5]{figures/emulator/eff_bits.png}
\caption{Emulated \muon~ detection efficiency as a function of the \ph~ background rate for different VMM3a bits configurations and pull-up currents, for \cpad~ close to the QL1 prototype values.
}
\label{fig: efficiency bits}
\end{figure}

\subsection{Monte Carlo simulation}
\label{subsec: detector emulator MC}

In order to test the validity of our hypothesis on the possible sources of inefficiency (see section~\ref{subsubsec: efficiency measurement}), we compared efficiency measurements with a Monte Carlo (MC) simulation. The inputs to the simulation were the measured ToT distribution and the \ph~ and \muon~ spectra. The signal jitter was considered negligible. The simulation was done by generating photon events at random times. Each event caused a dead-time t$\mathrm{_{dead}}$= ToT + 60~ns. If another signal was generated during dead-time, the latter would be extended accordingly. The \muon~ efficiency was calculated by checking the state of the system at a rate of 1~kHz. If the check occurred during dead-time, the event would be considered inefficient.
The comparison between emulated and MC results are presented in figure~\ref{fig: efficiency MC} for the QL1-like configuration with different \cpi~ values.
The MC simulation reproduces the results quite well, indicating that we could identify the main causes of inefficiency in the linear range (see section~\ref{subsubsec: efficiency measurement}). The emulated inefficiency for \cpi~= 470~pF could not be well reproduced, supporting the hipothesis that it is mainly caused by deeply saturated events, which were not included into the simulation. 

\begin{figure}[htbp]
\centering
\includegraphics[scale=0.5]{figures/emulator/eff_MC.png}
\caption{The comparison between emulated and MC results for the QL1-like configuration with different \cpi~ values.
}
\label{fig: efficiency MC}
\end{figure}

==> section_introduction.tex <==
\section{Introduction}
\label{sec: intro}

The Large Hadron Collider (LHC) at CERN is expected to be upgraded to the High-Luminosity LHC (HL-LHC) by 2029.  As it's name suggests, the HL-LHC is expected to achieve instantaneous luminosities around $5-7.5 \times 10^{34}$ cm$^{-2}$ s$^{-1}$.  This represents a more than $3-4$ fold increase in the instantaneous luminosity compared to what has been achieved in Run 2.  

All else equal, the increase in the instantaneous luminosity corresponds to a similar increase in background rates; mostly from low energy photons and neutrons. The latter, having large elastic cross section, bounce  in the detector cavern and generate random background signal long (order of microseconds) after their production in the collision. We refer to this collective diffuse gas of long-lived neutral particles as "cavern background". Previous measurements of cavern background using the ATLAS monitored drift tube (MDT) system have found that up to 65\% of hits in the MDTs come from a long-lived component with a half-life of 50 microseconds~\cite{NSW_TDR}.

At HL-LHC luminosities, we expect background rates of up to 15 kHz/cm$^2$ in the innermost end-cap region of the ATLAS muon spectrometer~\cite{NSW_TDR}. This region of the muon spectrometer, called the Small Wheel, is the part of the muon system that is to closest to the beam-line. % As such, we expect the highest rate of background, with the background rate growing exponentially as the distance to the beam line decreases as shown in figure 2.2 of Ref.~\cite{NSW_TDR}.
The background rate scaled with detector area corresponds to a maximum of 1 MHz per detector channel~\cite{NSW_TDR}.  The previous small wheel detectors cannot operate efficiently at such high rates and as such, 
%\begin{figure}[h!]
%\centering % \begin{center}/\end{center} takes some additional vertical space
%\includegraphics[width=.6\textwidth,trim=0 6 0 0,clip]{figures/intro/RateVsR.png}
%\caption{\label{fig:LHCrate} The measured background rate vs $r$~(taken from \cite{NSW_TDR}). The background hit rate increases exponentially with decreasing $r$. {\color{red}{Is this plot really useful? I think a plot about the predicted background rate at $5 \times 10^{34}$ will be more useful, the current plot is for very low instantanesous luminosity.}} }
%\end{figure}
A New Small Wheel (NSW) upgrade~\cite{NSW_TDR} is needed. The small-strip Thin Gap Chamber (sTGC) is one of two detector technologies used for this upgrade. %Both the detector and the electronics need to be able to operate efficiently in this high background environment. 
In this article, we summarize the results of multiple tests of sTGC detector and electronics at high rates.  

The paper is organized as follows. Section~\ref{sec: setup} describes the sTGC detector and its front-end electronics. 
Section~\ref{sec: TB October} covers the results of the first test beam of the detector in a high background rate environment in October 2018.  This test beam was the first measurement of detector efficiency as a function of background rate and found that the drop in efficiency at high rates can be fully parameterized by an exponential decay function with a single parameter: the electronics dead-time. 
Section \ref{sec: GIF++ analysis} covers on the measurements of the efficiency loss at high rate and the electronics dead-time with different input charge filters.  We also measured the dead-time when the front-end ASIC is set to operate in the trigger mode, which incurs less dead-time than the readout mode. These measurements were performed in March 2019.
Conclusions are drawn in section~\ref{sec: conclusion}.
%Section \ref{sec: detector emulation} covers the results of studies that seeks to mimic the input charge distribution measured in the test beam data in section \ref{sec: TB October} using a pulse generator.  This emulation study provides a more controlled environment to measure the relationship between the electronics dead-time and the charge per hit input into the amplifier. 

%{\color{red}{I feel that these paragraphs can be described in the conclusion section. Here we just introduce the sections and experiments we performed.

%The measurements are found to be consistent with one another.  The efficiency decreases with increasing background rate according to an exponential decay.  The rate of decay can be parameterized by a single parameter, the electronics dead-time. The dead-time increases with increasing input charge as the analog circuit must dump the input charge after every hit and recover to baseline before being ready for another hit.  

%These measurements of the relationship between efficiency at high rates, dead-time, and input charge per hit allowed us to set the optimal value for the pi-network filter that is placed in front of every sTGC pad input channel. The filter decreases the input charge per hit and minimizes the incurred dead-time and at the same time, allows enough input charge to separate signal from background.

%The present measurements also provide a more complete picture of the expected sTGC efficiency at HL-LHC rates and recommendation for sTGC electronics settings when operating at high rates.
%}
%}

\section{Experimental Setup}
\label{sec: setup}
\subsection{The sTGC Detector and Electronics}
\label{sec: intro_sTGC}

The sTGC is a multi-wire proportional chamber composed of a plane of gold-plated tungsten wire anodes sandwiched by two cathode planes as shown in figure \ref{fig: sTGC_Detector}. The wire diameter is 50 $\mu$m, the pitch size is 1.8 mm, and the wire-to-cathode distance is 1.4 mm. 

High voltage (typically 2,800~V) will be applied between the cathode and anode forming a strong electric field within the gas gap.  The electric field will be most concentrated around the wires. sTGC chambers are normally operated in a CO$_2$ and n-pentane gas mixture, which molecules can be ionized by the passage of energetic charged particles. The liberated primary electrons and ions will drift along the electric field lines to the anode and cathodes, respectively.  The primary electrons will be multiplied in an electron avalanche process as they approach the wires due to the strong electric field around them.  The charge motion of the electron-ion pairs formed in the avalanche is capacitively coupled to the cathode planes and anode wires.  The induced currents on the anode and cathode are in-turn read-out as signals. 

The cathodes are composed by two planes. A graphite-epoxy layer coated on FR4 faces the wires and serves for slow charge evacuation. The resistive layer and cathode-anode gap form an RC circuit that limits the speed of charge dispersion to ground, reducing the intensity of occasional discharges. The thickness of the graphite layer is 10 $\mu$m and its resistivity is in the order of 100 k$\Omega$ to 1 M$\Omega$. On the FR4 external side a copper plane is segmented either in pads or strips, which serve as signal pickup electrodes. The dimension of the readout elements changed with the position and with sTGC model. The large pads are used to quickly determine a region of interest for triggering.  The strips are used for determining the precise hit location and have a pitch size of 3.2 mm.

Four sTGC gaps are stacked together to form a quadruplet. This allows implementing different logic coincidence schemes in the trigger to optimize efficiency and background rejection.
In this work we describe results from two quadruplet models, namely QL1 and QS2.

\begin{figure}[h!]
\centering
\includegraphics[width=0.55\textwidth]{figures/sTGCDiag.png}
\caption{\protect A diagram of the sTGC detector (taken from \cite{sTGC_Proceeding}).  The wire anode is sandwiched between the pad and strip cathode planes.}
\label{fig: sTGC_Detector}
\end{figure}

%Important sTGC detector parameters are given in table \ref{tab: sTGC_Detector}.

%\begin{table}
%\centering
%    \begin{tabular}{p{6cm}|p{2cm}}
%    \hline \hline
%    \multicolumn{2}{c}{sTGC Geometrical and physical parameters}\\
%    \hline
%    wire-to-cathode pitch& 1.4 [mm]\\
%    \hline
%    wire-to-wire pitch & 1.8 [mm]\\
%    \hline
%    wire diameter & 50 [$\mu$m]\\
%    \hline
%    strip pitch & 3.2 [mm]\\
%    \hline
%    Graphite layer thickness & 10 [$\mu$m]\\
%    \hline
%    Q1 Graphite surface resistivity & 100 k$\Omega/\square$\\    \hline
%    Q2/Q3 Graphite surface resistivity & 200 k$\Omega/\square$\\
%    \hline \hline
%\end{tabular}
%    \caption{Detector parameters}
%    \label{tab: sTGC_Detector}
%\end{table}

The sTGC uses two front-end boards called the pad front-end board (pFEB) and the strip front-end board (sFEB) to read out the sTGC pads and strips, respectively~\cite{sTGCFEB}. The VMM3a ASIC described in section \ref{sec: intro_VMM} is the primary ASIC for the sTGC system each with 64 electronics channels.  A pFEB has three VMM3as, two reading the cathode pad channels signal and one reading the wire channels for the secondary coordinate measurement.  An sFEB has eight VMM3as to read out more than 400 strips on each detector layer. 
Each front-end board also has a Readout Controller (ROC) ASIC~\cite{ROC_Spec}, multiple Trigger Data Serializer (TDS) ASICs~\cite{TDS_Spec}, and a Slow Control Adapter (SCA) ASIC~\cite{SCA_Manual}.  These ASICs are used for data readout, sending trigger and slow control data, respectively.

The back-end DAQ system consist of a FPGA-based system called the miniDAQ system.  We use a KC705 Xilinx Kintex-7 FPGA evaluation board with a FSM-to-miniSAS adapter board to allow connections to the front-end boards. Each miniDAQ board is capable of timing-trigger-control, configuring, calibrating, and reading out up to eight front-end boards. The output data is sent via Ethernet and written to disk on a PC. % A diagram of the DAQ setup can be seen in figure~\ref{fig: miniDAQ}.  

%\begin{figure}[h!]
%\centering
%\includegraphics[scale=0.6]{figures/GIF_Setup/miniDAQ.png}
%\caption{\protect The miniDAQ system used to control and readout the front-end boards. }
%\label{fig: miniDAQ}
%\end{figure}

\subsection{The VMM3a Front-End ASIC}
\label{sec: intro_VMM}

The VMM3a is the primary front-end ASIC for the sTGC system~\cite{VMM_Spec}. It features 64 channels each with an amplifier, shaper, discriminator and a peak detector.  A 10-bit ADC is used to measure the precise charge of the hit, a 8-bit TDC measures the precise time of the hit, and a fast 6-bit ADC is used to quickly measure charge information that can be used for triggering.  

%A block diagram of the VMM3a can be seen in figure~\ref{fig: VMM_BlockDiagram}.

%\begin{figure}[h!]
%\centering
%\includegraphics[width=0.7\textwidth]{figures/GIF_Setup/vmm_blockdiagram.png}
%\caption{\protect Block diagram of the VMM3a ASIC, the primary front-end ASIC for the New Small Wheel~(taken from \cite{VMM_Spec}) }
%\label{fig: VMM_BlockDiagram}
%\end{figure}

The ASIC also contains digital logic including data buffering, trigger matching and event building. All hits within a 200~ns window of the received trigger will be packaged into an event and sent as an output data packet to the ROC ASIC.  

In parallel to the readout chain mentioned above, some information about all hits digitized by the VMM3a will be output via a direct output to the trigger chain without the need to receive a trigger.  The trigger chain sends less information about each hit than the readout chain, according to different operation modes.  For example, the time-over-threshold (ToT) information, a simple yes or no for when a pulse crosses threshold, can be sent for pad triggering.  For strips, the fast 6-bit ADC charge information is sent instead of the 10-bit ADC.  The sending of this quick but rough information is critical to forming a region of interest and constructing fast trigger segments that are then used by ATLAS trigger system to determine whether or not to read out the entire event.

%\subsection{The VMM3a Channel Reset Procedure}
%\label{sec: intro_VMM_Reset}

Figure \ref{fig: VMM_Reset} shows the VMM3a channel reset procedure in different operation modes.  The peak of the VMM3a analog output is reached after a time which depends on the ASIC peaking time and on the detector signal shape. The 10-bit ADC begins digitizing at the peak of the pulse. Studies using a detector emulation method as input to the ASIC show that this is around $60-70$ ns for a VMM3a peaking time setting of 50 ns and $35-40$ ns for a peaking time setting of 25 ns~\cite{DetEmulation}.    The digitization completes after a configurable amount of 10-bit ADC conversion time ($200-380$ ns).  Another 30 ns is needed for the channel to reset itself.  In this mode, this comes to a total reset time which is around 300 ns~\cite{VMM_Spec}.

In a different configurable setting, the VMM3a channel is reset as soon as the fast 6-bit ADC is complete.  The 6-bit ADC conversion time is configurable to be between 25 ns and 68.75 ns.  The same 30 ns reset time is needed after the completion of the 6-bit ADC digitization.  This gives a total of $\sim$125 ns but this is most likely optimistic as the analog pulse must also recover back to the baseline before the VMM3a channel is ready for another hit.  For a moderate amount of charge such as 6 pC the recovery time for the analog pulse can be around 60 ns.  This combined with a rise time of $60-70$ ns gives the same order of 130 ns that is expected from the 6-bit ADC reset mode~\cite{DetEmulation}. For large charge deposits due to the tail of the energy deposited by a minimum ionizing particle or neutral particles such as photons and long-lived neutrons the recovery time can be as long as $1-2$ microseconds. In this case, the time with which the analog pulse takes to recover back below the threshold is therefore the limiting factor regardless of the ADC's recovery if the operating mode is not that of the 10-bit ADC.

Finally a ToT operation mode may be selected where the channel resets after the pulse crosses back below the threshold, without waiting for the completion of any ADC conversion. Also in this case, the limiting factor is the recovery of the analog pulse.

% The diagrams are from an internal document
\begin{figure}[h!]
\centering
\begin{subfigure}[b]{0.48\textwidth}
\includegraphics[width=\textwidth]{figures/GIF_Setup/10BitADC_Reset.png}
\caption{}
\label{subfig: 10BitADC_Rest}
\end{subfigure}
\begin{subfigure}[b]{0.4\textwidth}
\includegraphics[width=\textwidth]{figures/GIF_Setup/ToT_Reset.png}
\caption{}
\label{subfig: ToT_Reset}
\end{subfigure}

\caption{ The VMM3a Channel reset procedure in different operation modes~\cite{VMM_Spec}. \ref{subfig: 10BitADC_Rest} shows the reset procedure for the 10-bit ADC mode.  A separate setting for resetting when the faster 6-bit ADC is also possible. \ref{subfig: ToT_Reset} shows the reset procedure for the ToT operation mode.  }
\label{fig: VMM_Reset}
\end{figure}

\subsection{The Pi-Network Filter and Pull Up Resistor on the VMM3a input}
\label{sec: intro_PiNetwork}

The signal from the sTGC detector consists of three components.  A fast component comes from the fast moving electrons in the electron avalanche drifting towards the wire anode in the first 20~ns.  A slow component with the same polarity happens in the next tens of microseconds due to ions drifting towards the cathode. The ion drift signal continues until the ions reach the cathode plane.  The third component can be as slow as a few milliseconds and it is induced by the charge movement in the resistive layer after ions landing. This component has opposite polarity with respect to the first two. %A plot of the simulated input current from an sTGC channel is given in figure \ref{fig: sTGC_Signal} (the third component is not visible here)\cite{VMM_Spec}. 
A measurement of average sTGC current and charge signals is shown in figure~\ref{fig: emulator signal}~\cite{DetEmulation}, showing the fast and slow components.



%\begin{figure}[h!]
%\centering
%\includegraphics[scale=0.6]{figures/GIF_Setup/sTGC_Signal.png}
%\caption{Simulated distribution of the signal for the sTGC detector.  Y-axis is current on the detector channel and y-axis is time in microseconds. The fast immediate electron component and the slow ion component of the signal can be seen~(taken from \cite{NSW_TDR}). }
%\label{fig: sTGC_Signal}
%\end{figure}

\begin{figure}[h!]
\centering
%\subfloat[Complete signal]{
%\includegraphics[scale=0.4]{figures/emulator/emulator_signal_all}
%\label{subfig: complete signal}
%}
%\\
%\subfloat[Positive current]{
\includegraphics[scale=0.4]{figures/emulator/emulator_signal_positive_1}
%\label{subfig: positive current}
%}
\caption{The average sTGC integrated charge signal shape (in blue) and its derivative (in red, corresponding to the current signal)~\cite{DetEmulation}.
}
\label{fig: emulator signal}
\end{figure}

At high rates, the long ion tail from many hits will be superimposed upon one another to form a constant input current into the amplifier.  This is especially true for the sTGC detector which expect to have a high background rate of long-lived neutral particles such as low energy neutrons.  The VMM3a has a baseline recovery circuit to counter-act this low frequency input and maintain the stability of the baseline at high rates. 

A single cavern background hit can deposit as much as 50 pC of charge in one sTGC pad according to simulation \cite{VMM_Spec}, which can saturate the ASIC's amplifier. For this reason, an additional input filter circuit called the pi-network (shown in figure~\ref{subfig: PiNetwork}) was designed to attenuate the signal of the sTGC pad channels.  The pi-network acts as a charge divider, splitting the charge left in the detector channel with that of its own capacitor.  At the same time, the two bias resistors connected to the 1.2V power rail act as a current source to counter-act the constant input current due to the ion tail, thereby acting as an aid to the VMM3a's baseline recovery circuit.  

 The pi-network and detector channel capacitors are in series and the charge accumulated will be divided among the two according to their capacitance.  In addition to reducing detector noise and background hits, the pi-network capacitor also attenuates the muon signal.  The capacitance and attenuation must be optimized. % to maintain the size of the muon signal but limit the amount of charge from highly ionizing photons and neutrons that can saturate the VMM3a's amplifier. 
 The rough estimate of the attenuation factor ($f$) of the pi-network is given by eq.~\ref{eqn: pi-attenuation}:
\begin{equation}
    f = \frac{C_{p}}{C_{p}+C_{\text{detector}}}
    \label{eqn: pi-attenuation}
\end{equation}
where $C_p$ is the capacitance of the pi-network and $C_{\text{detector}}$ is the capacitance of the detector channel. 
 The true equation is much more complicated and frequency dependent because of the nature of the RC network but this represents a ball-park estimation of $f$.


A pull-up resistor (shown in figure~\ref{subfig: StripPullUp}) is added to the sTGC strips channels.  We expect the charge from a single hit to be split across more than three strips and so the input charge per strip channel is less than that of a pad channel.  The pull-up resistor is able to draw a constant counter-acting current that flows counter to that of the long-ion tail and thereby partially cancelling it. A resistance that is too small will correspond to a too large input current at low rates with no long-ion tail current to cancel. The current through the resistor will itself overwhelm the baseline recovery circuit at low background rates rendering the amplifier non-functional. Therefore an optimization is also needed.  Simulation of the ASIC performance suggest that a charge divider such as that used for the pads is not needed here.

%Both the pad pi-network and strip pull up resistor diagrams are shown in figure \ref{fig: PiNetworkDiagram}.

\begin{figure}[h!]
\centering
 \begin{subfigure}[b]{0.45\textwidth}
\includegraphics[width=\textwidth]{figures/GIF_Setup/PiNetworkDiagram.png}
\caption{}
\label{subfig: PiNetwork}
 \end{subfigure}
\qquad
 \begin{subfigure}[b]{0.45\textwidth}
\includegraphics[width=\textwidth]{figures/GIF_Setup/StripPullUpDiagram.png}
\caption{}
\label{subfig: StripPullUp}
\end{subfigure}
\caption{ \ref{subfig: PiNetwork}: The pi-Network filter placed in between a sTGC pad and the input to the VMM3a amplifier.  \ref{subfig: StripPullUp}: The pull-up resistor placed in between a sTGC strip and the input to the VMM3a amplifier.  }
\label{fig: PiNetworkDiagram}
\end{figure}

%The measurements in this paper explain how to quantify the effect of these circuits and how we determined the optimal values of the pi network capacitor and the strip pull up resistor.

